Paragraph-level Commonsense Transformers with Recurrent Memory

Human understanding of narrative texts requires making commonsense inferences beyond what is stated explicitly in the text. A recent model, COMET, can generate such implicit commonsense inferences along several dimensions such as pre- and post-conditions, motivations, and mental states of the participants. However, COMET was trained on commonsense inferences of short phrases, and is therefore discourse-agnostic. When presented with each sentence of a multi-sentence narrative, it might generate inferences that are inconsistent with the rest of the narrative. We present the task of discourse-aware commonsense inference. Given a sentence within a narrative, the goal is to generate commonsense inferences along predefined dimensions, while maintaining coherence with the rest of the narrative. Such large-scale paragraph-level annotation is hard to get and costly, so we use available sentence-level annotations to efficiently and automatically construct a distantly supervised corpus. Using this corpus, we train PARA-COMET, a discourse-aware model that incorporates paragraph-level information to generate coherent commonsense inferences from narratives. PARA-COMET captures both semantic knowledge pertaining to prior world knowledge, and episodic knowledge involving how current events relate to prior and future events in a narrative. Our results show that PARA-COMET outperforms the sentence-level baselines, particularly in generating inferences that are both coherent and novel.

==> figures/loss.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lll}
\toprule
\textbf{Model} & \textbf{Train} & \textbf{Val}  \\ 
\midrule
Memory-less & 2.27 & 2.63 \\
Memory-less w/o pretraining & 2.23 & 2.63 \\
Memory-augmented & 2.18 & 2.62 \\
\bottomrule
\end{tabular}
\caption{Average training and validation losses.}
\label{table:train_val_loss}
\end{table}

==> figures/weakly_supervised_examples.tex <==
\begin{table*}
\begin{center}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{  l l c c c} 
\toprule
Narrative  & Inference & Relevant? & LM score \\
\midrule
\textbf{Natalie's favorite movie is The Wizard of Oz}... & PersonX wanted: to see the film & \correct & -3.384     \\
I was at the grocery store...\textbf{I see the lines were very long}... & PersonX then feels: relieved & \incorrect &  -3.408 \\ 
Jim wanted to learn Spanish. \textbf{He tried taking a class}...  & PersonY/Others want: to catch up & \incorrect & -3.602 \\
\textbf{Our building had a summer bbq party today.} The manager took photos... & PersonX wants: to enjoy the party & \correct & -3.915 \\
Chris realizes that he rarely watches cable TV anymore. \textbf{He calls}...\textbf{to cancel}... & PersonX wanted: to be a good customer & \incorrect & -3.952 \\
My grandparents lived in Alabama. We used to travel there...\textbf{I miss traveling there}... & PersonX is seen as: sad & \correct & -3.518 \\
\bottomrule
\end{tabular}
}
\caption{Examples from the distantly supervised dataset. We highlight the most relevant (i.e. potentially contradictory or supporting) sections in the story for each inference being considered. LM score shows the average token log probability. Inferences are marked as relevant (\correct) or irrelevant (\incorrect).} %\ronan{Highlight the sentence used to generate the inference?}\ronan{Instead of "Relevance", should we use "story-level consistency", to be consistent with the naming? and maybe include sentence-level consistency? How should we interpret the LM scores? Was the goal to support our choice of coherence measure?}\saadia{Right, and we specifically ask annotators if the inferences are relevant}}
\label{table:ws_examples}
\end{center}
\end{table*}
